Path Diffuser: Diffusion Model for Data-Driven Traffic Simulator

Simulating diverse and realistic traffic scenarios is critical for developing and testing autonomous planning. Traditional rule-based planners lack diversity and realism, while learning-based simulators often replay, forecast, or edit scenarios using historical agent trajectories. However, they struggle to generate new scenarios, limiting scalability and diversity due to their reliance on fully annotated logs and historical data. Thus, a key challenge for a learning-based simulator's performance is that it requires agents' past trajectories and pose information in addition to map data, which might not be available for all agents on the road.Without which, generated scenarios often produce unrealistic trajectories that deviate from drivable areas, particularly under out-of-distribution (OOD) map scenes (e.g., curved roads). To address this, we propose Path Diffuser (PD): a two-stage, diffusion model for generating agent pose initializations and their corresponding trajectories conditioned on the map, free of any historical context of agents' trajectories. Furthermore, PD incorporates a motion primitive-based prior, leveraging Frenet frame candidate trajectories to enhance diversity while ensuring road-compliant trajectory generation. We also explore various design choices for modeling complex multi-agent interactions. We demonstrate the effectiveness of our method through extensive experiments on the Argoverse2 Dataset and additionally evaluate the generalizability of the approach on OOD map variants. Notably, Path Diffuser outperforms the baseline methods by 1.92x on distribution metrics, 1.14x on common-sense metrics, and 1.62x on road compliance from adversarial benchmarks.

==> sections/acknowledgement.tex <==

\section*{Acknowledgment}
This work is supported in part by the Natural Sciences and Engineering Research Council of Canada (NSERC) and Canada Foundation for Innovation - John R. Evans Leaders Fund (CFI JELF).

